Learning Student-Friendly Teacher Networks for Knowledge Distillation

We propose a novel knowledge distillation approach to facilitate the transfer of dark knowledge from a teacher to a student. Contrary to most of the existing methods that rely on effective training of student models given pretrained teachers, we aim to learn the teacher models that are friendly to students and, consequently, more appropriate for knowledge transfer. In other words, at the time of optimizing a teacher model, the proposed algorithm learns the student branches jointly to obtain student-friendly representations. Since the main goal of our approach lies in training teacher models and the subsequent knowledge distillation procedure is straightforward, most of the existing knowledge distillation methods can adopt this technique to improve the performance of diverse student models in terms of accuracy and convergence speed. The proposed algorithm demonstrates outstanding accuracy in several well-known knowledge distillation techniques with various combinations of teacher and student models even in the case that their architectures are heterogeneous and there is no prior knowledge about student models at the time of training teacher networks.

==> experiments_cite.tex <==
%!TEX root = icml_sftn.tex

\section{Experiments}
\label{sec:experiments}
We now evaluate the performance of SFTN in comparison to existing methods and analyze the characteristics of SFTN in various aspects. 
We first describe our experiment setting in Section~\ref{sub:experiment}.
% Then, we present the comparison results between SFTN and the conventional teacher networks with respect to classification accuracy in various knowledge distillation algorithms in Section~\ref{sub:benchmark}.
Then, we present the comparison results between SFTN and the standard teacher networks with respect to classification accuracy in various knowledge distillation algorithms in Section~\ref{sub:benchmark}.
The results from ablative experiments for SFTN and transfer learning are discussed in Section~\ref{sub:ablation_study} and  \ref{sub:transfer_learning}.
% Section~\ref{sub:comp_training} compares KD~\cite{KD} training of SFTN and standard knowledge distillation. 
Also we measure similarity between distillation student and teacher, Section~\ref{sub:similarity} shows results of similarity. 

\subsection{Experiment Setting}
\label{sub:experiment}
We perform evaluation on multiple well-known datasets including ImageNet~\cite{IMAGENET}. CIFAR-100~\cite{cifar09}, and STL10~\cite{STL10}.
For the experiment, we select several different backbone networks such as ResNet~\cite{resnet}, WideResNet~\cite{WRN}, VGG~\cite{vggnet}, ShuffleNetV1~\cite{ShuffleNetv1}, and ShuffleNetV2~\cite{ShuffleNetv2}. 

For comprehensive evaluation, we adopt various knowledge distillation techniques, which include KD~\cite{KD}, FitNets~\cite{FitNet}, AT~\cite{AT}, SP~\cite{sp}, VID~\cite{vid}, RKD~\cite{RKD}, PKT~\cite{pkt}, AB~\cite{ABdistill}, FT~\cite{FT}, CRD~\cite{CRD}, SSKD~\cite{SSKD}, and OH~\cite{OH}. 
Among these methods, the feature distillation methods~\cite{FitNet,AT,sp,vid,RKD,pkt,ABdistill,FT,OH} conduct joint distillation with conventional KD~\cite{KD} during student training, which results in higher accuracy in practice than the feature distillation only.
We have reproduced the results from the existing methods using the implementations provided by the authors.
% PyTorch~\cite{pytorch} .


\begin{table*}[t]
\centering
\caption{Comparisons between SFTN and the standard teacher models on CIFAR-100 dataset when the architectures of the teacher-student pairs are homogeneous. 
%Diff, +KD and bold denotes difference between SFTN and TN(conventional teacher), combine distillation of conventional KD~\cite{KD}, and best result of row, respectively. 
In all the tested algorithms, the student models distilled from the teacher models given by SFTN outperform  the ones trained from the standard teacher models. All the reported accuracies in this table is computed by the outputs of 3 independent runs. }
\label{table:homogeneous_teacher_student}
\scalebox{0.82}{%
\begin{tabular}{c||ccc|ccc|ccc|ccc}
Models (Teacher/Student)                   & \multicolumn{3}{c|}{WRN40-2/WRN16-2} & \multicolumn{3}{c|}{WRN40-2/WRN40-1} & \multicolumn{3}{c|}{ResNet32x4/ResNet8x4} & \multicolumn{3}{c}{VGG13/VGG8} \\
Teacher   training method                  & Standard    & SFTN     & $\Delta$   & Standard    & SFTN     & $\Delta$   & Standard      & SFTN      & $\Delta$     & Standard  & SFTN   & $\Delta$  \\ \hline\hline
Teacher   Accuracy                         & 76.30        & 78.2     &            & 76.30        & 77.62    &            & 79.25         & 79.41     &              & 75.38     & 76.76  &           \\
Student   accuracy w/o KD                  &             & 73.41    &            &             & 72.16    &            &               & 72.38     &              &           & 71.12  &           \\ \hline
KD~\cite{KD}        & 75.46       & 76.25    & $+$0.79       & 73.73       & 75.09    & $+$1.36       & 73.39         & 76.09     & $+$2.70          & 73.41     & 74.52  & $+$1.11      \\
FitNets~\cite{FitNet}  & 75.72       & 76.73    & $+$1.01       & 74.14       & 75.54    & $+$1.40        & 75.34         & 76.89     & $+$1.55         & 73.49     & 74.38  & $+$0.89      \\
AT~\cite{AT}         & 75.85       & 76.82    & $+$0.97       & 74.56       & 75.86    & $+$1.30        & 74.98         & 76.91     & $+$1.93         & 73.78     & 73.86  & $+$0.08      \\
SP~\cite{sp}           & 75.43       & 76.77    & $+$1.34       & 74.51       & 75.31    & $+$0.80        & 74.06         & 76.37     & $+$2.31         & 73.37     & 74.62  & $+$1.25      \\
VID~\cite{vid}        & 75.63       & 76.79    & $+$1.16       & 74.21       & 75.76    & $+$1.55       & 74.86         & 77.00        & $+$2.14         & 73.81     & 74.73  & $+$0.92      \\
RKD~\cite{RKD}          & 75.48       & 76.49    & $+$1.01       & 73.86       & 75.11    & $+$1.25       & 74.12         & 76.62     & $+$2.50          & 73.52     & 74.48  & $+$0.96      \\
PKT~\cite{pkt}          & 75.71       & 76.57    & $+$0.86       & 74.43       & 75.49    & $+$1.06       & 74.70          & 76.57     & $+$1.87         & 73.60      & 74.51  & $+$0.91      \\
AB~\cite{ABdistill}   & 70.12       & 70.76    & $+$0.64       & 74.38       & 75.51    & $+$1.13       & 74.73         & 76.51     & $+$1.78         & 73.20      & 74.67  & $+$1.47      \\
FT~\cite{FT}         & 75.6        & 76.51    & $+$0.91       & 74.49       & 75.11    & $+$0.62       & 74.89         & 77.02     & $+$2.13         & 73.64     & 74.30   & $+$0.66      \\
CRD~\cite{CRD}       & 75.91       & 77.23    & $+$1.32       & 74.93       & 76.09    & $+$1.16       & 75.54         & 76.95     & $+$1.41         & 74.26     & 74.86  & $+$0.60       \\
SSKD~\cite{SSKD}     & 75.96       & 76.80     & $+$0.84       & 75.72       & 76.03    & $+$0.31       & 75.95         & 76.85     & $+$0.90          & 74.94     & 75.66  & $+$0.72      \\
OH~\cite{OH}         & 76.00          & 76.39    & $+$0.39        & 74.79       & 75.62    & $+$0.83       & 75.04         & 76.65     & $+$1.61         & 73.94     & 74.72  & $+$0.78      \\ \hline
Best                                       & 76.00          & 77.23    & $+$1.23       & 75.72       & 76.09    & $+$0.37       & 75.95         & 77.02     & $+$1.07         & 74.94     & 75.66  & $+$0.72 \\ \hline   
\end{tabular}%
}
\end{table*}

\begin{table*}[t]
\centering
\caption{Comparisons between SFTN and the standard teacher models on CIFAR-100 dataset when the architectures of the teacher-student pairs are heterogeneous. 
%Diff, +KD and bold denotes difference between SFTN and TN(conventional teacher), combine distillation of conventional KD~\cite{KD}, and best result of row, respectively. 
In all the tested algorithms, the student models distilled from the teacher models given by SFTN outperform  the ones trained from the standard teacher models. All the reported accuracies in this table is computed by the outputs of 3 independent runs. }
\label{table:heterogeneous_teacher_student}
\scalebox{0.82}{%
\begin{tabular}{c||ccc|ccc|ccc|ccc}
Models (Teacher/Student)  & \multicolumn{3}{c}{ResNet32x4/ShuffleV1} & \multicolumn{3}{c}{ResNet32x4/ShuffleV2} & \multicolumn{3}{c}{ResNet50/VGG8} & \multicolumn{3}{c}{WRN40-2/ShuffleV2} \\
Teacher   training method & Standard       & SFTN       & $\Delta$       & Standard       & SFTN        & $\Delta$      & Standard     & SFTN     & $\Delta$    & Standard      & SFTN       & $\Delta$     \\ \hline\hline
Teacher   Accuracy        & 79.25          & 80.03      &            & 79.25          & 79.58       &           & 78.70         & 82.52    &         & 76.30          & 78.21      &          \\
Student   accuracy w/o KD	    &  	&71.95	& 	&	&73.21	&	&	&71.12   &         &    &73.21  &	    \\ \hline
KD~\cite{KD}                        & 74.26          & 77.93      & $+$3.67      & 75.25          & 78.07       & $+$2.82      & 73.82        & 74.92    & $+$1.10     & 76.68         & 78.06      & $+$1.38     \\
FitNets~\cite{FitNet}                    & 75.95          & 78.75      & $+$2.80       & 77.00             & 79.68       & $+$2.68      & 73.22        & 74.80     & $+$1.58    & 77.31         & 79.21      & $+$1.90     \\
AT~\cite{AT}                        & 76.12          & 78.63      & $+$2.51      & 76.57          & 78.79       & $+$2.22      & 73.56        & 74.05    & $+$0.49    & 77.41         & 78.29      & $+$0.88     \\
SP~\cite{sp}                        & 75.80           & 78.36      & $+$2.56      & 76.11          & 78.38       & $+$2.27      & 74.02        & 75.37    & $+$1.35    & 76.93         & 78.12      & $+$1.19     \\
VID~\cite{vid}                       & 75.16          & 78.03      & $+$2.87      & 75.70           & 78.49       & $+$2.79      & 73.59        & 74.76    & $+$1.17    & 77.27         & 78.78      & $+$1.51     \\
RKD~\cite{RKD}                       & 74.84          & 77.72      & $+$2.88      & 75.48          & 77.77       & $+$2.29      & 73.54        & 74.70     & $+$1.16    & 76.69         & 78.11      & $+$1.42     \\
PKT~\cite{pkt}                       & 75.05          & 77.46      & $+$2.41      & 75.79          & 78.28       & $+$2.49      & 73.79        & 75.17    & $+$1.38    & 76.86         & 78.28      & $+$1.42     \\
AB~\cite{ABdistill}                        & 75.95          & 78.53      & $+$2.58      & 76.25          & 78.68       & $+$2.43      & 73.72        & 74.77    & $+$1.05    & 77.28         & 78.77      & $+$1.49      \\
FT~\cite{FT}                        & 75.58          & 77.84      & $+$2.26      & 76.42          & 78.37       & $+$1.95      & 73.34        & 74.77    & $+$1.43    & 76.80          & 77.65      & $+$0.85     \\
CRD~\cite{CRD}                      & 75.60           & 78.20       & $+$2.60        & 76.35          & 78.43       & $+$2.08      & 74.52        & 75.41    & $+$0.89    & 77.52         & 78.81      & $+$1.29     \\
SSKD~\cite{SSKD}                      & 78.05          & 79.10       & $+$1.05       & 78.66          & 79.65       & $+$0.99      & 76.03        & 76.95    & $+$0.92    & 77.81         & 78.34      & $+$0.53     \\
OH~\cite{OH}                      & 77.51          & 79.56      & $+$2.05       & 78.08          & 79.98       & $+$1.90      & 74.55        & 75.95    & $+$1.40     & 77.82         & 79.14      & $+$1.32     \\ \hline
Best                      & 78.05          & 79.56      & $+$1.51        & 78.66          & 79.98       & $+$1.32      & 76.03        & 76.95    & $+$0.92    & 77.82         & 79.21      & $+$1.39     \\ \hline 
\end{tabular}%
}
\end{table*}


\subsection{Main Results}
\label{sub:benchmark}

To show effectiveness of SFTN, we incorporate SFTN into various existing knowledge distillation algorithms and evaluate accuracy.
We present implementation details and experimental results on CIFAR-100~\cite{cifar09} and ImageNet~\cite{IMAGENET} datasets.
%With these results, we can prove that our SFTN work well in various environment.



\subsubsection{CIFAR-100} 

CIFAR-100~\cite{cifar09} is one of the common benchmark datasets for the evaluation of knowledge distillation algorithms. 
It consists of 50K training images and 10K testing images in 100 classes. 
We select 12 state-of-the art distillation methods to compare accuracy of SFTN with the standard teacher network. 
To show the generality of the proposed approach, 8 pairs of teacher and student models have been tested in our experiment.
The experiment setup for CIFAR-100 is identical to the one performed in CRD\footnote{https://github.com/HobbitLong/RepDistille}; most experiments employ the SGD optimizer with learning rate 0.05, weight decay 0.0005 and momentum 0.9 while learning rate is set to 0.01 in ShuffleNet experiments. 
%We trained all the networks for 240 epochs. Learning rate is multiplied by 0.1 at 150, 180, 210. 
The hyper-parameters for the loss function are set as $\lambda_\text{T}=1$, $\lambda_\text{R}^\text{CE}=1$, $\lambda_\text{R}^\text{KL}=3$, and ${\tau=1}$.

Table~\ref{table:homogeneous_teacher_student} and \ref{table:heterogeneous_teacher_student} demonstrates the full results on the CIFAR-100 dataset.
Table~\ref{table:homogeneous_teacher_student} presents distillation performance of all the compared algorithms when the architecture styles of teacher and student pairs are same while Table~\ref{table:heterogeneous_teacher_student} shows distillation performance of different architectural style teacher-student pairs. 
Both tables clearly present that SFTN is consistently better than the standard teacher network in all experiments. 
The average difference between standard teacher and SFTN is 1.49\% points, and the average difference between best student accuracy of standard teacher and SFTN is 1.06\% points.
Figure~\ref{fig:comp_best_student} illustrates the accuracies of the best student models of both teacher networks given teacher and student architecture pairs. 
Despite the small capacity of the student networks, the 5 best student models of SFTN outperform the standard teachers while the only one best student of the standard teacher shows higher accuracy than its teacher.

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{./images/fig3.png}
\end{center}
\vspace{-0.3cm}
  \caption{Accuracy comparison of the best students from SFTN with the standard teacher. The 5 best student models of SFTN outperform the standard teachers while the only one best student of the standard teacher shows higher accuracy than its teacher.}
\label{fig:comp_best_student}
\end{figure*}



\subsubsection{ImageNet}

\begin{table}[t]
\centering
\caption{Top-1 and Top-5 validation accuracy on ImageNet.}
\label{table:imagenet_result}
\scalebox{0.8}{%
\begin{tabular}{c||ccc|ccc}
\begin{tabular}[c]{@{}c@{}}Models\\(Teacher/Student)\end{tabular}  & \multicolumn{6}{c}{ResNet50/ResNet34}                \\ \hline
                          & \multicolumn{3}{c|}{Top-1}  & \multicolumn{3}{c}{Top-5} \\ 
% Teacher\\training method & Standard & SFTN   & $\Delta$& Standard & SFTN  & $\Delta$  \\ \hline\hline
Teacher training & Stan. & SFTN   & $\Delta$& Stan. & SFTN  & $\Delta$  \\ \hline\hline
Teacher Acc.      & 76.45   & 77.43  &       & 93.15   & 93.75 &       \\
Stu. Acc. w/o KD &          & 73.79  &       &          & 91.74 &       \\ \hline
KD~\cite{KD}                         & 73.55    & 74.14  & $+$0.59  & 91.81     & 92.21 & $+$0.40 \\
FitNets~\cite{FitNet}                     & 74.56   & 75.01  & $+$0.45 & 92.31    & 92.51 & $+$0.20   \\
SP~\cite{sp}                        & 74.95   & 75.53 & $+$0.58 & 92.54    & 92.69  & $+$0.15 \\
CRD~\cite{CRD}                       & 75.01   & 75.39  & $+$0.38 & 92.56    & 92.67 & $+$0.11 \\
OH~\cite{OH}                        & 74.56    & 75.01  & $+$0.45  & 92.36    & 92.56  & $+$0.20 \\ \hline
Best                      & 75.01   & 75.53 & $+$0.52 & 92.56    & 92.69  & $+$0.13 \\ \hline
\end{tabular}%
}
\end{table}

ImageNet~\cite{IMAGENET} is a large-scale dataset constructed for image classification. 
The dataset consists of 1.2M training images and 50K validation images for 1K classes. 
We adopt the standard Pytorch ImageNet training setup\footnote{https://github.com/pytorch/examples/tree/master/imagenet} for this experiment. 
The optimization is given by SGD with learning rate 0.1, weight decay 0.0001 and momentum 0.9. 
%{\color{blue}Training epochs of experiments is set to 100. Learning rate is multiplied by 0.1 at 30, 60, 90.}
The coefficients of individual loss terms are set as $\lambda_\text{T}=1$, $\lambda_\text{R}^\text{CE}=1$ $\lambda_\text{R}^\text{KL}=1$ and $\tau=1$. 
We conduct the ImageNet experiment for 5 different knowledge distillation methods with one pair of teacher and student models, where teacher models based on ResNet50 distillate knowledge to ResNet34 student networks. 

As presented in Table~\ref{table:imagenet_result}, SFTN consistently outperforms the standard teacher network in all settings.
Also, the best student accuracy of SFTN achieves higher top-1 accuracy than standard teacher model by approximately 0.5\%. 
This results implies that the proposed SFTN works well on large datasets as well.


\subsection{Effect of Hyperparameters}
\label{sub:ablation_study}
SFTN computes the KL-divergence loss to minimize the difference between the softmax outputs of teacher and student branches, which involves two relevant hyperparameters, temperature of the softmax function, ${\tau}$, and weight for KL-divergence loss term, $\lambda_\text{R}^\text{KL}$.
This section discusses the impact and trade-off issue of the two hyperparameters.
In particular, we present our observations that learning student-friendly representations is indeed helpful to improve the accuracy of student models while maximizing the performance of SFTN may be suboptimal for knowledge distillation.

% \begin{table*}[!htb]
%     \caption{Effects of varying ${\tau}$}
%     \label{table:varying_tau}
%       \centering
%         \scalebox{0.8}{%      
%         \begin{tabular}{c|ccccc|c|ccccc|c}
%          & \multicolumn{6}{c|}{Teacher Accuracy}  & \multicolumn{6}{c}{KD~\cite{KD} Accuracy}   \\ \hline                                                                     
%         Teacher              & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} \\ 
%         Student              & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1        & VGG8           &   & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1        & VGG8           &                     \\ \hline 
%         Standard             & 79.25          & 79.25          & 76.30           & 76.30           & 75.38          & 77.30   & 74.31          & 75.25          & 75.28          & 73.56          & 73.31          & 74.34            \\
%         SFTN &	&	&	&	&	&	&	&	&	&	&	& \\
%          ${\tau}$=1              & 81.19          & 80.26          & 78.23          & 78.14          & 76.44          & 78.85 & 76.05 & 77.18 & 76.30           & 74.75 & 73.06           & \textbf{75.58}               \\
%          ${\tau}$=5              & 81.23          & 81.56          & 79.22          & 78.31          & 77.40           & 79.54 & 75.36          & 75.59          & 76.31 & 73.64          & 74.61 & 75.10               \\
%          ${\tau}$=10             & 81.27          & 81.98 & 78.81          & 78.38          &77.48 & 79.58  & 74.47          & 75.93          & 75.85          & 73.62          & 73.91          & 74.76              \\
%          ${\tau}$=15             & 81.89 & 81.74          & 79.27 & 78.63 & 77.15          & \textbf{79.74} & 74.78          & 75.65          & 75.79          & 73.49          & 74.33          & 74.81     \\
%          ${\tau}$=20             & 81.60           & 81.70           & 78.84          & 78.45          & 77.37          & 79.59   & 74.62          & 75.88          & 75.82          & 74.03          & 74.41          & 74.95      \\ \hline         
%         \end{tabular}%
%         }
 
% \end{table*}


\begin{table*}[!htb]
    % \caption{Effects of varying ${\tau}$ {\color{blue}in SFTN}. The student accuracy is fairly stable over a wide range of the parameter. Note that the accuracies of SFTN and student are rather inversely correlated, which implies that the maximization of teacher models is not necessarily idea for knowledge distillation.}

    \caption{Effects of varying ${\tau}$ in the knowledge distillation via SFTN. The student accuracy is fairly stable over a wide range of the parameter. Note that the accuracies of SFTN and student are rather inversely correlated, which implies that the maximization of teacher models is not necessarily idea for knowledge distillation.}
    \label{table:varying_tau}
      \centering
        \scalebox{0.82}{%      
        \begin{tabular}{c||cccc|c||cccc|c}
         & \multicolumn{5}{c||}{Accuracy of SFTN}  & \multicolumn{5}{c}{Student accuracy by KD~\cite{KD}}   \\ \hline                                                                     
        Teacher              & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} \\ 
        Student              & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1        &   & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1       &                     \\ \hline 
%        Standard             & 79.25          & 79.25          & 76.30           & 76.30                     & 77.30   & 74.31          & 75.25          & 75.28          & 73.56                    & 74.34            \\
%        SFTN &  &  &  &  & &  &  &   &   &   \\
         ${\tau}$=1              & 81.19  & 80.26 & 78.23 & 78.14 & 78.85           & 76.05 & 77.18 & 76.30  & 74.75  & \textbf{75.58}               \\
         ${\tau}$=5              & 81.23  & 81.56 & 79.22 & 78.31 & 79.54           & 75.36 & 75.59 & 76.31  & 73.64  & 75.10               \\
         ${\tau}$=10             & 81.27 & 81.98 & 78.81 & 78.38 & 79.58            & 74.47 & 75.93 & 75.85  & 73.62  & 74.76              \\
         ${\tau}$=15             & 81.89 & 81.74 & 79.27 & 78.63 & \textbf{79.74} & 74.78 & 75.65 & 75.79  & 73.49 & 74.81     \\
         ${\tau}$=20             & 81.60 & 81.70 & 78.84  & 78.45 & 79.59           & 74.62 & 75.88 & 75.82  & 74.03 & 74.95      \\ \hline         
        \end{tabular}%
        }
 
\end{table*}

\begin{table*}[!htb]
% \caption{Effects of varying $\lambda_\text{R}^\text{KL}$. The student accuracy is fairly stable over a wide range of the parameter. Note that the accuracies of SFTN and student are not correlated while the accuracy gaps of the two model drops as $\lambda_\text{R}^\text{KL}$ increases.}
% \caption{Effects of varying $\lambda_\text{R}^\text{KL}$ {\color{blue}in SFTN}. The accuracies of SFTN and student are not correlated while the accuracy gaps of the two model drops as $\lambda_\text{R}^\text{KL}$ increases.}
\caption{Effects of varying $\lambda_\text{R}^\text{KL}$ in the knowledge distillation via SFTN. The accuracies of SFTN and student are not correlated while the accuracy gaps of the two model drops as $\lambda_\text{R}^\text{KL}$ increases.}
\label{table:varying_s_kl}
 \centering
\scalebox{0.82}{%
\begin{tabular}{c||cccc|c||cccc|c}
         & \multicolumn{5}{c||}{Accuracy of SFTN}  & \multicolumn{5}{c}{Student accuracy by KD~\cite{KD}}   \\ \hline                                                                     
        Teacher              & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} & ResNet32x4     & ResNet32x4     & WRN40-2        & WRN40-2        & \multirow{2}{*}{AVG} \\ 
        Student              & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1        &   & ShuffleV1      & ShuffleV2      & WRN16-2        & WRN40-1       &                     \\ \hline 
%        Standard             & 79.25          & 79.25          & 76.30           & 76.30                     & 77.78   & 74.31          & 75.25          & 75.28          & 73.56                    & 74.60            \\
%        SFTN &  &  &  &  & &  &  &   &   &   \\
       
        $\lambda_\text{R}^\text{KL}$=1            & 81.19      & 80.26      & 78.23   & 78.14  & \textbf{79.46}      & 76.05      & 77.18      & 76.30    & 74.75  & 76.07               \\
        $\lambda_\text{R}^\text{KL}$=3          & 78.70       & 79.80       & 77.83   & 77.57   & 78.48               & 77.36      & 78.56      & 76.20    & 74.71   & \textbf{76.71}       \\
        $\lambda_\text{R}^\text{KL}$=6            & 78.29      & 78.29      & 77.28   & 76.05  & 77.48               & 77.33      & 77.70       & 76.02   & 74.67   & 76.43              \\
        $\lambda_\text{R}^\text{KL}$=10         & 73.02      & 75.01      & 75.03   & 73.51   & 74.14               & 75.57      & 76.62      & 74.19   & 73.08   & 74.87            \\ \hline
        Standard           & 79.25      & 79.25      & 76.30   & 76.30   & 77.78       & 74.31      & 75.25     & 75.28  & 73.56 & 74.60 \\ \hline
        %   \\
\end{tabular}%
}
\end{table*}


\paragraph{Temperature of softmax function} 
The temperature parameter, denoted by ${\tau}$, controls the softness of $\mathbf{q}_\text{T}$ and $\mathbf{q}_\text{R}^{i}$; as ${\tau}$ gets higher, the output of the softmax function becomes smoother.
The accuracy of the student model given by KD via SFTN is fairly consistent.
Table~\ref{table:varying_tau} also shows that the performance of SFTNs and student models is rather inversely correlated.
In other words, a loosely optimized teacher model turns out to be more effective for knowledge distillation according to this ablation study.
%{\color{blue}which may be related to model capacity gap issue.}
%Therefore ${\tau}$ may need to be optimized depending on the teacher-student architecture pair. 
%Here, it needs to be stressed that making higher accuracy of SFTN does not guarantee higher accuracy of student network. 
%Results in Table~\ref{table:varying_tau} show accuracies of SFTN and distilled student can be in trade-off relationship depending on the hyper parameter ranges.

\paragraph{Weight for KL-divergence loss} 
$\lambda_\text{R}^\text{KL}$ is a parameter that makes $\mathbf{q}_\text{T}$ similar to $\mathbf{q}_\text{R}^{i}$, and consequently facilitates knowledge distillation.
However, it affects the accuracy of teacher network negatively.
Table~\ref{table:varying_s_kl} shows that the average accuracy gaps between SFTNs and student models drops gradually as $\lambda_\text{R}^\text{KL}$ increases.
% In particular, when $\lambda_\text{R}^\text{KL}=10$, the student model even outperforms its corresponding SFTN, which shows that the similarity between teacher and student networks plays an important role in the distillation process. 
%{\color{blue} Student accuracy rises and then falls, due to improved similarity and decreased teacher network accuracy.
One interesting observation is the student accuracy via SFTN with $\lambda_\text{R}^\text{KL}=10$ compared to its counterpart via the standard teacher; even though the standard teacher network is more accurate than SFTN by a large margin, its corresponding student accuracy is lower than that of SFTN.
%It shows the trade-off between the performances of the two models.
%SFTN is of lower accuracy than standard teacher, but SFTN distilled student shows better accuracy than the standard teacher when $\lambda_\text{R}^\text{KL}$=10. 
More details about similarity between student and teacher network is discussed in Section~\ref{sub:similarity}. 



\subsection{Transferability}
\label{sub:transfer_learning}
%

The goal of transfer learning is to obtain versatile representations that adapt well on unseen datasets.
To investigate transferability of the student models distilled from SFTN, we perform experiments to transfer the student features learned on CIFAR-100 to STL10~\cite{STL10} and TinyImageNet~\cite{TinyImageNet}. 
The representations of the examples in CIFAR-100 are obtained from the last student block and frozen  during transfer learning, and then we make the features fit to the target datasets using linear classifiers attached to the last student block.

Table~\ref{table:transfer_result} presents transfer learning results on 5 different knowledge distillation algorithms using ResNet32$\times$4 and ShuffleV2 as teacher and student, respectively. 
Our experiments show that the accuracy of transfer learning on the student models derived from SFTN is consistently better than the students associated with the standard teacher. 
The best student accuracy of SFTN even outperforms that of the standard teacher by 3.02\% points on STL10 and 4.06\% points on TinyImageNet.
%
\begin{table*}[t]
\centering
\caption{The accuracy of student models on STL10 and TinyImageNet by transferring knowledge from the models trained on CIFAR-100.}
\label{table:transfer_result}
\scalebox{0.82}{%
\begin{tabular}{c||ccc|ccc}
Models (Teacher/Student)  & \multicolumn{6}{c}{ResNet32x4/ShuffleV2}           \\ \hline
% \multirow{2}{*}{}         & \multicolumn{3}{c|}{\multirow{2}{*}{CIFAR100-\textgreater{}STL10}}       & \multicolumn{3}{c}{\multirow{2}{*}{CIFAR100-\textgreater{}TinyImageNet}} \\
%                           & \multicolumn{3}{c}{}                                                    & \multicolumn{3}{c}{}                                                     \\
         & \multicolumn{3}{c|}{CIFAR100 $\rightarrow$ STL10}       & \multicolumn{3}{c}{CIFAR100 $\rightarrow$ TinyImageNet} \\
%\begin{tabular}[c]{@{}c@{}}Teacher \\ Training \end{tabular}                          & Standard             & SFTN                      & $\Delta$                 & Standard              & SFTN                      & $\Delta$                 \\ \hline\hline
~~~Teacher training method~~~                      & ~Standard~             & ~SFTN~                      & ~~$\Delta$~~                 & ~Standard~              & ~~SFTN~~                      & ~$\Delta$~                 \\ \hline\hline
%\begin{tabular}[c]{@{}c@{}}Teacher\\Accuracy\end{tabular}        & 69.81              & 76.84                   & 7.03                & 31.25                 & 40.16                     & 8.91                 \\
% Teacher accuracy        & 69.81              & 76.84                   & 7.03                & 31.25                 & 40.16                     & 8.91                 \\
Teacher accuracy        & 69.81              & 76.84                   &                 & 31.25                 & 40.16                     &                 \\
% \begin{tabular}[c]{@{}c@{}}Student\\Accuracy w/o KD\end{tabular} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{70.18} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{33.81} & \multicolumn{1}{l}{} \\ \hline
%\begin{tabular}[c]{@{}c@{}}Student\\Accuracy w/o KD\end{tabular} &          & 70.18  &       &          & 33.81 &       \\ \hline
Student accuracy w/o KD &          & 70.18  &       &          & 33.81 &       \\ \hline
KD~\cite{KD}                         & 67.49              & 73.81                     & $+$6.32                 & 30.45                 & 37.81                     & $+$7.36                 \\
SP~\cite{sp}                        & 69.56              & 75.01                   & $+$5.45                 & 31.16                 & 38.28                     & $+$7.12                 \\
CRD~\cite{CRD}                       & 71.70                 & 75.80                      &$+$4.10                  & 35.50                  & 40.87                     & $+$5.37                 \\
SSKD~\cite{SSKD}                      & 74.43               & 77.45                     & $+$3.02                 & 38.35                 & 42.41                     & $+$4.06                 \\
OH~\cite{OH}                        & 72.09              & 76.76                   & $+$4.67                 & 33.52                 & 39.95                     & $+$6.43                 \\ \hline
Best                      & 74.43               & 77.45                     & $+$3.02                 & 38.35                 & 42.41                     & $+$4.06                \\ \hline
\end{tabular}%
}
\end{table*}



% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=0.75\linewidth, height=1.3\linewidth]{./images/comparison_distillation.png}
% \end{center}
%   \caption{knowledge distillation training graph. Conventional KD\cite{KD} is used for distillation method. SFTN resnet32x4 converges faster and show higher test accuracy than conventional resnet32x4. }
% \label{fig:comp_training}
% \end{figure}

% \subsection{Comparison of Knowledge Distillation Training}
% \label{sub:comp_training}
% Conventional KD~\cite{KD} calculates KL loss for minimize soft distribution between teacher and student, and Figure ~\ref{fig:comp_training} (a) present result of training KL Loss of Conventional KD. In Figure ~\ref{fig:comp_training} (a), KL loss of SFTN converges much faster than standard knowledge distillation. In SFTN strategy, teacher trains with student branch before distillation for easier feature, So teacher representation of SFTN is more similar to student than standard knowledge distillation. Since more similar teacher representation of SFTN, student of SFTN can minimize soft distribution between teacher and student much faster than student of standard knowledge distillation. Also Figure~\ref{fig:comp_training} (b) shows that test acc of SFTN student is much higher than 
% standard knowledge distillation student.


\subsection{Similarity}
\label{sub:similarity}
Similarity between student and teacher network is an important measure for knowledge distillation tasks considering student network is basically trying to resemble similar output of teacher network. 
Here, we use KL-divergence and CKA~\cite{cka} as metrics of similarity between student and teacher network, where lower KL-divergence and higher CKA indicate higher similarity.
%Especially KL-div=0, CKA=1 mean both networks show same behavior. 

\begin{table}[t]
\centering
\caption{Similarity measurements between teachers and students on the CIFAR-100 test set. Higher CKA and lower KL indicate that the representations given by two models are more similar. }
\label{table:similarity}
\scalebox{0.8}{%
\begin{tabular}{c|cc|cc}
Models (Teacher/Student)  & \multicolumn{4}{c}{ResNet32x4/ShuffleV2}         \\ \hline
                          & \multicolumn{2}{c|}{KL-divergence} & \multicolumn{2}{c}{CKA} \\
Teacher   training method & Standard     & SFTN    & Standard      & SFTN    \\ \hline\hline
KD~\cite{KD}                        & 1.10          & 0.47    & 0.88          & 0.95    \\
FitNets~\cite{FitNet}                    & 0.79         & 0.38    & 0.89          & 0.95    \\
AT~\cite{AT}                        & 0.86         & 0.42    & 0.88          & 0.95    \\
SP~\cite{sp}                        & 0.95         & 0.45    & 0.89          & 0.95    \\
VID~\cite{vid}                       & 0.88         & 0.45    & 0.88          & 0.95    \\
RKD~\cite{RKD}                       & 0.88         & 0.47    & 0.88          & 0.95    \\
PKT~\cite{pkt}                       & 0.89         & 0.46    & 0.89          & 0.95    \\
AB~\cite{ABdistill}                        & 0.92         & 0.47    & 0.88          & 0.95    \\
FT~\cite{FT}                        & 0.80          & 0.42    & 0.88          & 0.95    \\
CRD~\cite{CRD}                        & 0.81         & 0.43    & 0.88          & 0.95    \\
SSKD~\cite{SSKD}                      & 0.54         & 0.26    & 0.92          & 0.97    \\ 
OH~\cite{OH}                        & 0.85         & 0.37    & 0.90          & 0.96    \\ \hline
AVG                       & 0.86         & 0.42    & 0.89          & 0.95   \\ \hline
\end{tabular}%
}
\end{table}
%
Table~\ref{table:similarity} presents the similarities between the representations of a ResNet32$\times$4 teacher and a ShuffleV2 student given by various algorithms on the CIFAR-100 test set.
The results show that the distillation from SFTN always gives higher similarity to the student model with respect to the teacher network; SFTN reduces KL-divergence by 50\% in average while improving average CKA by 6\% compared to the standard teacher network.
%SFTN consistently trains more similar student than standard teacher’s knowledge distillation. 
Since SFTN is trained with student branches to obtain student-friendly representations via a KL-divergence loss, the improved similarity is quite natural. 
%We also show how the distillation process differs in the similarity aspect.
Figure~\ref{fig:comp_training}(a) illustrates the KL-divergence loss for the distillation of SFTN converges faster and is optimized better than the knowledge distillation from the standard teacher network.
%, which means student network gets similar to SFTN faster and finally behaves more like SFTN. 
Consequently, we observe higher test accuracy of SFTN as shown in Figure~\ref{fig:comp_training}(b).
%
\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  % include first image
  \includegraphics[width=.85\linewidth]{./images/fig4_a.png}  
  \subcaption{KL-divergence loss during training on CIFAR-100.\vspace{0.1cm}} 
  \label{fig:comp_training_a}
\end{subfigure} 
\begin{subfigure}{.5\textwidth}
  \centering
  % include second image
  \includegraphics[width=.85\linewidth]{./images/fig4_b.png}  
  \subcaption{Test accuracy on CIFAR-100.}
  \label{fig:comp_training_b}
\end{subfigure}

\caption{Visualization of some training and testing curves, where ResNet32$\times$4 and ShuffleV2 are employed as the teacher and student networks, respectively.
SFTN converges faster and show improved test accuracy than the standard teacher models.}
\label{fig:comp_training}
\end{figure}

==> references_item.tex <==
% \begin{thebibliography}{10}

% \bibitem{KD}
% Geoffrey Hinton, Oriol Vinyals, and Jeffrey Dean.
% \newblock {Distilling the Knowledge in a Neural Network}.
% \newblock In {\em NeurIPS Deep Learning and Representation Learning Workshop},
%   2015.

% \bibitem{kang2020towards}
% Minsoo Kang, Jonghwan Mun, and Bohyung Han.
% \newblock Towards oracle knowledge distillation with neural architecture
%   search.
% \newblock In {\em AAAI}, 2020.

% \bibitem{mirzadeh2019improved}
% Seyed-Iman Mirzadeh, Mehrdad Farajtabar, Ang Li, and Hassan Ghasemzadeh.
% \newblock Improved knowledge distillation via teacher assistant: Bridging the
%   gap between student and teacher.
% \newblock In {\em AAAI}, 2020.

% \bibitem{DML}
% Ying Zhang, Tao Xiang, Timothy~M Hospedales, and Huchuan Lu.
% \newblock {Deep Mutual Learning}.
% \newblock In {\em CVPR}, 2018.

% \bibitem{KDCL}
% Qiushan Guo, Xinjiang Wang, Yichao Wu, Zhipeng Yu, Ding Liang, Xiaolin Hu, and
%   Ping Luo.
% \newblock Online knowledge distillation via collaborative learning.
% \newblock In {\em CVPR}, 2020.

% \bibitem{PCL}
% Guile Wu and Shaogang Gong.
% \newblock Peer collaborative learning for online knowledge distillation.
% \newblock In {\em arXiv 2006.04147}, 2020.

% \bibitem{Chen2017LearningEO}
% Guobin Chen, Wongun Choi, Xiangdong Chen, Tony~X. Han, and Manmohan~Krishna
%   Chandraker.
% \newblock {Learning Efficient Object Detection Models with Knowledge
%   Distillation}.
% \newblock In {\em NeurIPS}, 2017.

% \bibitem{facemodel}
% Ping Luo, Zhenyao Zhu, Ziwei Liu, Xiaogang Wang, and Xiaoou Tang.
% \newblock {Face Model Compression by Distilling Knowledge from Neurons}.
% \newblock In {\em AAAI}, 2016.

% \bibitem{reidentification}
% Ancong Wu, Wei{-}Shi Zheng, Xiaowei Guo, and Jian{-}Huang Lai.
% \newblock Distilled person re-identification: Towards a more scalable system.
% \newblock In {\em CVPR}, 2019.

% \bibitem{styletransfer}
% Huan Wang, Yijun Li, Yuehai Wang, Haoji Hu, and Ming{-}Hsuan Yang.
% \newblock Collaborative distillation for ultra-resolution universal style
%   transfer.
% \newblock In {\em CVPR}, 2020.

% \bibitem{tinybert}
% Xiaoqi Jiao, Yichun Yin, Lifeng Shang, Xin Jiang, Xiao Chen, Linlin Li, Fang
%   Wang, and Qun Liu.
% \newblock Tinybert: Distilling {BERT} for natural language understanding.
% \newblock In {\em arXiv:1909.10351}, 2019.

% \bibitem{mclkd}
% Jonghwan Mun, Kimin Lee, Jinwoo Shin, and Bohyung Han.
% \newblock {Learning to Specialize with Knowledge Distillation for Visual
%   Question Answering}.
% \newblock In {\em NeurIPS}, 2018.

% \bibitem{distillbert}
% Victor Sanh, Lysandre Debut, Julien Chaumond, and Thomas Wolf.
% \newblock Distilbert, a distilled version of {BERT:} smaller, faster, cheaper
%   and lighter.
% \newblock {\em CoRR}, 2019.

% \bibitem{distill_response}
% Siddhartha Arora, Mitesh~M. Khapra, and Harish~G. Ramaswamy.
% \newblock On knowledge distillation from complex networks for response
%   prediction.
% \newblock In Jill Burstein, Christy Doran, and Thamar Solorio, editors, {\em
%   NAACL}, 2019.

% \bibitem{action_recognition}
% Fida~Mohammad Thoker and Juergen Gall.
% \newblock Cross-modal knowledge distillation for action recognition.
% \newblock In {\em ICIP}, 2019.

% \bibitem{radio_signals}
% Mingmin Zhao, Tianhong Li, Mohammad~Abu Alsheikh, Yonglong Tian, Hang Zhao,
%   Antonio Torralba, and Dina Katabi.
% \newblock Through-wall human pose estimation using radio signals.
% \newblock In {\em CVPR}, 2018.

% \bibitem{zhou2020domain}
% Brady Zhou, Nimit Kalra, and Philipp Kr{\"a}henb{\"u}hl.
% \newblock Domain adaptation through task distillation.
% \newblock In {\em ECCV}, 2020.

% \bibitem{FitNet}
% Adriana Romero, Nicolas Ballas, Samira~Ebrahimi Kahou, Antoine Chassang, Carlo
%   Gatta, and Yoshua Bengio.
% \newblock {FitNets: Hints for Thin Deep Nets}.
% \newblock In {\em ICLR}, 2015.

% \bibitem{OH}
% Byeongho Heo, Jeesoo Kim, Sangdoo Yun, Hyojin Park, Nojun Kwak, and Jin~Young
%   Choi.
% \newblock A comprehensive overhaul of feature distillation.
% \newblock In {\em ICCV}, 2019.

% \bibitem{AT}
% Sergey Zagoruyko and Nikos Komodakis.
% \newblock {Paying More Attention to Attention: Improving the Performance of
%   Convolutional Neural Networks via Attention Transfer}.
% \newblock In {\em ICLR}, 2017.

% \bibitem{FT}
% Jangho Kim, SeongUk Park, and Nojun Kwak.
% \newblock {Paraphrasing Complex Network: Network Compression via Factor
%   Transfer}.
% \newblock In {\em NeurIPS}, 2018.

% \bibitem{RKD}
% Wonpyo Park, Dongju Kim, Yan Lu, and Minsu Cho.
% \newblock {Relational Knowledge Distillation}.
% \newblock In {\em CVPR}, 2019.

% \bibitem{CRD}
% Yonglong Tian, Dilip Krishnan, and Phillip Isola.
% \newblock Contrastive representation distillation.
% \newblock In {\em ICLR}, 2020.

% \bibitem{lan2018knowledge}
% Xu~Lan, Xiatian Zhu, and Shaogang Gong.
% \newblock {Knowledge Distillation by On-the-Fly Native Ensemble}.
% \newblock In {\em NeurIPS}, 2018.

% \bibitem{byot}
% Linfeng Zhang, Jiebo Song, Anni Gao, Jingwei Chen, Chenglong Bao, and Kaisheng
%   Ma.
% \newblock Be your own teacher: Improve the performance of convolutional neural
%   networks via self distillation.
% \newblock In {\em ICCV}, 2019.

% \bibitem{SSKD}
% Guodong Xu, Ziwei Liu, Xiaoxiao Li, and Chen~Change Loy.
% \newblock Knowledge distillation meets self-supervision.
% \newblock In {\em ECCV}, 2020.

% \bibitem{BAN}
% Tommaso Furlanello, Zachary~Chase Lipton, Michael Tschannen, Laurent Itti, and
%   Anima Anandkumar.
% \newblock Born-again neural networks.
% \newblock In {\em ICML}, 2018.

% \bibitem{RCO}
% Xiao Jin, Baoyun Peng, Yichao Wu, Yu~Liu, Jiaheng Liu, Ding Liang, Junjie Yan,
%   and Xiaolin Hu.
% \newblock Knowledge distillation via route constrained optimization.
% \newblock In {\em ICCV}, 2019.

% \bibitem{efficacykd}
% Jang~Hyun Cho and Bharath Hariharan.
% \newblock On the efficacy of knowledge distillation.
% \newblock In {\em ICCV}, 2019.

% \bibitem{IMAGENET}
% Olga Russakovsky, Jia Deng, Hao Su, Jonathan Krause, Sanjeev Satheesh, Sean Ma,
%   Zhiheng Huang, Andrej Karpathy, Aditya Khosla, Michael~S. Bernstein,
%   Alexander~C. Berg, and Fei{-}Fei Li.
% \newblock Imagenet large scale visual recognition challenge.
% \newblock {\em Int. J. Comput. Vis.}, 115(3):211--252, 2015.

% \bibitem{cifar09}
% Alex Krizhevsky.
% \newblock {Learning Multiple Layers of Features from Tiny Images}.
% \newblock Technical report, Citeseer, 2009.

% \bibitem{resnet}
% Kaiming He, Xiangyu Zhang, Shaoqing Ren, and Jian Sun.
% \newblock {Deep Residual Learning for Image Recognition}.
% \newblock In {\em CVPR}, 2016.

% \bibitem{WRN}
% Sergey Zagoruyko and Nikos Komodakis.
% \newblock Wide residual networks.
% \newblock In {\em BMVC}, 2016.

% \bibitem{vggnet}
% Karen Simonyan and Andrew Zisserman.
% \newblock {Very Deep Convolutional Networks for Large-Scale Image Recognition}.
% \newblock In {\em ICLR}, 2015.

% \bibitem{ShuffleNetv1}
% Xiangyu Zhang, Xinyu Zhou, Mengxiao Lin, and Jian Sun.
% \newblock Shufflenet: An extremely efficient convolutional neural network for
%   mobile devices.
% \newblock In {\em CVPR}, 2018.

% \bibitem{ShuffleNetv2}
% Mingxing Tan, Bo~Chen, Ruoming Pang, Vijay Vasudevan, Mark Sandler, Andrew
%   Howard, and Quoc~V. Le.
% \newblock Mnasnet: Platform-aware neural architecture search for mobile.
% \newblock In {\em CVPR}, 2019.

% \bibitem{sp}
% Frederick Tung and Greg Mori.
% \newblock Similarity-preserving knowledge distillation.
% \newblock In {\em ICCV}, 2019.

% \bibitem{vid}
% Sungsoo Ahn, Shell~Xu Hu, Andreas~C. Damianou, Neil~D. Lawrence, and Zhenwen
%   Dai.
% \newblock Variational information distillation for knowledge transfer.
% \newblock In {\em CVPR}, 2019.

% \bibitem{pkt}
% Nikolaos Passalis and Anastasios Tefas.
% \newblock Learning deep representations with probabilistic knowledge transfer.
% \newblock In {\em ECCV}, 2018.

% \bibitem{ABdistill}
% Byeongho Heo, Minsik Lee, Sangdoo Yun, and Jin~Young Choi.
% \newblock Knowledge transfer via distillation of activation boundaries formed
%   by hidden neurons.
% \newblock In {\em AAAI}, 2019.

% \bibitem{cka}
% Simon Kornblith, Mohammad Norouzi, Honglak Lee, and Geoffrey~E. Hinton.
% \newblock Similarity of neural network representations revisited.
% \newblock In {\em ICML}, 2019.

% \bibitem{hendrycks2019robustness}
% Dan Hendrycks and Thomas Dietterich.
% \newblock Benchmarking neural network robustness to common corruptions and
%   perturbations.
% \newblock In {\em ICLR}, 2019.

% \bibitem{STL10}
% Adam Coates, Andrew~Y. Ng, and Honglak Lee.
% \newblock An analysis of single-layer networks in unsupervised feature
%   learning.
% \newblock In {\em AISTATS}, 2011.

% \bibitem{TinyImageNet}
% http://tiny imagenet.herokuapp.com/.

% \end{thebibliography}












